Dynamic Simplex: Balancing Safety and Performance in Autonomous Cyber Physical Systems

Learning Enabled Components (LEC) have greatly assisted cyber-physical systems in achieving higher levels of autonomy. However, LEC's susceptibility to dynamic and uncertain operating conditions is a critical challenge for the safety of these systems. Redundant controller architectures have been widely adopted for safety assurance in such contexts. These architectures augment LEC "performant" controllers that are difficult to verify with "safety" controllers and the decision logic to switch between them. While these architectures ensure safety, we point out two limitations. First, they are trained offline to learn a conservative policy of always selecting a controller that maintains the system's safety, which limits the system's adaptability to dynamic and non-stationary environments. Second, they do not support reverse switching from the safety controller to the performant controller, even when the threat to safety is no longer present. To address these limitations, we propose a dynamic simplex strategy with an online controller switching logic that allows two-way switching. We consider switching as a sequential decision-making problem and model it as a semi-Markov decision process. We leverage a combination of a myopic selector using surrogate models (for the forward switch) and a non-myopic planner (for the reverse switch) to balance safety and performance. We evaluate this approach using an autonomous vehicle case study in the CARLA simulator using different driving conditions, locations, and component failures. We show that the proposed approach results in fewer collisions and higher performance than state-of-the-art alternatives.

==> ResponseLetter.tex <==
\setcounter{page}{1}
 \pagestyle{plain}
 \newcommand{\cAron}[1]{\todo[color=blue!10, linecolor=black!50]{\textcolor{black}{\textbf{Aron}: {#1}}}}
\newcommand{\cScott}[1]{\todo[color=green!10, linecolor=black!50]{\textcolor{black}{\textbf{Scott}: {#1}}}}
\newcommand{\Abhishek}[1]{\todo[color=orange!10, linecolor=black!50,inline]{\textcolor{black}{\textbf{Abhishek}: {#1}}}}
\setlength{\parskip}{\baselineskip}
\setlength{\parindent}{0pt}

\renewcommand{\revision}[1]{#1}


\begin{center}
\large{Response to Reviews}\\
\vspace{0.1in}
\large{\textbf{Dynamic Simplex: Balancing Safety and Performance in Autonomous Cyber Physical Systems}}\\
\vspace{0.1in}
%\textbf{Manuscript ID: TCPS-2020-0079}
\end{center}

\vspace{0.5in}
Dear Shepherd and Reviewers,

We thank you for your time and effort for providing constructive feedback on our manuscript. We have taken care to create a major revision that we feel addresses the reviewer comments. 
Below, we provide a detailed description of how we have addressed these comments. To help you with the verification of these changes, we have addressed each comment separately, and the most important changes in the major revision of our paper are typeset in \textcolor{blue}{blue~text}. 

%We are pleased to submit a major revision of our paper for consideration in the Transaction on Cyber-Physical Systems Special Issue on Artificial Intelligence and Cyber-Physical Systems. We thank the reviewers and editors for their constructive feedback on our previous submission. Below, we provide a detailed description of how we have addressed these comments in our revision. We have addressed each comment separately, and these changes are typeset in \textcolor{blue}{blue~text}. 

We thank you again for the time that you dedicated to our paper and look forward to hearing from~you.

Sincerely,
\newline
Baiting Luo, Shreyas Ramakrishna, Ava Pettet, Christopher Kuhn, Gabor Karsai, Ayan Mukhopadhyay
% \vspace{0.5in}

%\newpage
%---------------------------------------------------------------------
\section*{Response to Shepherd}

\reviewerComment{}{%
First, I would request a kind of ablation study.  Your reverse switch combines a non-myopic planner and a set of domain rules.  What is their relative contribution?  One way is to re-run your experiments, first, with a myopic switch and domain rules and, second, with the non-myopic planner and no domain rules.  Maybe you already have these results.  There may be other ways to tease these two aspects apart, I don't want to be too prescriptive.
The second request is a little more open-ended.  Ultimately, the paper needs a better discussion about balancing performance and safety.  Whether you call it dynamic simplex or not, this balance is what this line of work is after.  The consensus of the reviewers was that your work is rather too ad hoc for that, but it offers a useful step in the right direction.  That's where the discussion comes in.  Generally, one expects safety guarantees, which are hard to establish for data-driven techniques.  Would you argue that guarantees are not needed and evaluation is enough to show that the technique works in general, or do you expect to establish some soft of guarantees in future work (and, if so, what kind of guarantees you envision for this approach)?  How does one know when the balance is achieved?}

\response{%
Thank you for the feedback. As suggested, we have carefully revised the paper and incorporated all the reviewers' comments. To improve the paper, we have added additional content and experiments as listed below. This has increased the length of the appendix.}


The specific additions that we have made are as follows. 

\begin{enumerate}[noitemsep]
%\item \textbf{Title:}
%We have  updated the title from ``Efficient Out-of-Distribution Detection and Diagnosis using Disentangled Latent Representations'' to ``Efficient Out-of-distribution Detection Using Latent Space of $\beta$-VAE for Cyber-Physical Systems''. 
%\item \textbf{Introduction and Problem:} \cref{sec:intro} -  We have revised the contents of the introduction to set up the \ac{ood} detection problem and compare it to the state-of-the-art techniques. Further, we have clarified the problem specification in \cref{sec:problem}. Specific requirements for the detectors have been added as a list. Further, we have shown the effectiveness of our approach by formulating an online time series change detection problem as well. 
%\item \textbf{Partial Disentanglement}: We have clarified that we are interested in achieving partial disentanglement and not full disentanglement, which is very difficult to achieve for practical datasets.  Even partial disentanglement provides good detection capabilities as shown in \cref{Table:design-space}, and aid in \ac{ood} reasoning (See \cref{fig:confidence} and \cref{fig:nuImage-confidence}).
%\item \textbf{Background:} We have added a background section \cref{sec:background} which was missing in our previous version.  
\item \textbf{Ablation Study:} In \cref{appendix:ablation study}, we have added the results of the ablation study in \cref{fig:ablation}. We do an ablation study in four reverse-switching configurations: myopic switch with domain rules, myopic switch without domain rules, non-myopic switch with domain rules, non-myopic switch with domain rules. 

\item \textbf{Safety Guarantee:} We have updated \cref{sec:approach}, \cref{sec:surrogate}, and \cref{sec:conclusion} to state that the myopic selector driven by the surrogate model is an example of how to apply our approach. We’ll assume that the forward switching conditions will be provided when the approach is applied to real-world applications to guarantee safety further.

\item \textbf{Discussion of Balance:} We further explain how the system the balance is achieved in \cref{appendix:balance analysis}. Our approach is not ad-hoc to safety-critical systems but can also be applied to mission-critical systems. Depending on the goal of the system, the balance between safety and performance can be achieved by tuning the parameters in our utility functions.



%Generally, domain rules are applied when the system tries to perform reverse switching while it is not in a stable state (turning) or is in a complex environment (junction). Theoretically, more and different domain rules can reduce the number of infractions, but they may also compromise the system’s performance. 
%\item The \textbf{discussion} and the \textbf{related research} sections have been revised as well. Specifically these new references have been added: \cite{kohli2019enabling}, \cite{dubey2011model},\cite{szegedy2013deep}, \cite{nuimage}, \cite{hartsell2021resonate}, \cite{sundar2020out}, \cite{tran2017disentangled}, \cite{peng2017reconstruction}, \cite{jakab2020partial}, \cite{mathieu2019disentangling}, \cite{hutter2019automated}, ~\cite{welford1962note}, \cite{basseville1993detection}, \cite{seto1998simplex}, ~\cite{edwards2008elements}, ~\cite{fremont2019scenic}, ~\cite{msdl}, ~\cite{dejanovic2017textx}, \cite{pan2009survey}, ~\cite{long2015learning}, \cite{heinze2021conditional}, \cite{volpi2018generalizing}, \cite{wang2019characterizing},  \cite{devries2018learning}, \cite{lakshminarayanan2016simple}, \cite{geifman2018bias}, \cite{jha2019attribution}, \cite{sundararajan2017axiomatic}, \cite{makhzani2015adversarial}, \cite{beggel2019robust}.

% We have evised the data generation section to include a \acl{sdl} that is shown in \cref{Table:Train}. Further, we have clarified the distribution change between trained and test data. We have also added \cref{fig:latent-plots}. It explains the effectiveness of our approach of selecting most informative latent variables. 

% \textbf{Experiments:} In \cref{sec:experiments} we demonstrate our approach for an \ac{av} example in CARLA simulation and a real-world automotive dataset called nuImages. In \cref{sec:system-setup} we have revised the data generation section to include a \acl{sdl} that is shown in \cref{Table:Train}. In \cref{sec:detector-design} we have added revised contents of the latent variable mapping paragraph and the results table in \cref{Table:avgkl}. We have also introduced \cref{fig:latent-plots} to explain out approach of selecting most informative latent variables. In \cref{sec:experiments} we have added additional experiments and revised its content. Specifically, we have rewritten \cref{sec:runtime-ood} to clearly explain our experiments for runtime \ac{ood} detection. \cref{fig:change-point} are plots from new experiments added to this revision of the work. \cref{sec:design-evaluation} has been a new content added to evaluate or design approach and the results are reported in \cref{Table:design-space}. \cref{sec:nuimage} discuss the newly added experiments for nuImages dataset. Further, \cref{sec:discussion} has been revised to better suite the new contents of the revised paper.
\end{enumerate}




%(3) \cref{sec:problem} - We have also revised a few paragraphs of the problem formulation section to include a new problem and included a requirements paragraph. 








%Finally, we have revised the related work in \cref{sec:RW} to include the papers suggested by the reviewers. 




%---------------------------------------------------------------------
%\clearpage
\section*{Response to Reviewer \#1}

\reviewerComment{}{%
Nevertheless, after reading the paper I was left particularly concerned with the approach used in this work, which really looks at odds with the nature of the simplex paradigm. Learning-based algorithms (either based on surrogate models for the forward switch or based on generative models for the backward switch) are used for switching between controllers. This however questions the applicability of the proposed methods to safety-critical systems, as the switching algorithms (as well as the corresponding monitors), which are obviously crucial for the safety of the system, may be very hard to verify.
}

\response{% 
We have updated \cref{sec:approach}, \cref{sec:surrogate}, and \cref{sec:conclusion} to state that the myopic selector driven by the surrogate model is an example of how to apply our approach. We’ll assume that the forward switching conditions will be provided when the approach is applied to real-world applications to guarantee safety further.}


\reviewerComment{}{Finally, the extensive use of historical data to ensure the safety of the system, and in particular to deal with system faults, conflicts with and ignores the rich literature on functional safety. This is at odds with ISO26262 mentioned in the paper. For instance, does the ISO26262 accepts fault models for hardware components such as cameras that entirely based on historical data?}

\response{%
Such a question is not explicitly discussed in ISO26262, but a typical way to construct the fault model is to classify the fault into six different categories: “safe fault,” “single point fault,” “residual fault,” “detected multi-point fault,” “perceived multi-point fault,” and “latent multi-point” fault. And determining the probability of a given fault being of a specific type is done by taking a large enough sample of faults and measuring their distribution between the various types~\cite{ISO}. Similar to this idea, our work trains a surrogate model with a large number of simulations to evaluate the risk of the camera fault. 
}


\reviewerComment{}{What happens if the historical data are poisoned?
}

\response{%
If any transitions in the environment model or the poisoned historical data are detected, we can simply update the underlying models with the most up-to-date information available at hand. This is also one of the advantages of using the online planning method. 
}

% \paperQuote{\revision{\textbf{Implementation}: We provide an approach (See \cref{fig:approach}) to design \ac{bvae} based latent space detectors. It has design-time steps of data partitioning, latent space encoding, latent variable mapping (discussed in this section), and runtime anomaly detection (discussed in \cref{sec:anomaly-detection}). These steps work as follows: \underline{First}, we divide the multi-labeled datasets into partitions based on the variance in the feature values. A partition consists of images with one feature having higher variance in its values, irrespective of changes in the others. \underline{Second}, we generate a latent space encoding using a \ac{bvae}, which provides a gating parameter $\beta$ to control the feature information in the latent space. The value of $\beta$ and the number of latent variables ($n$) influence the level of latent space interpretability. To find the optimal hyperparameter combination we propose a heuristic that uses the \ac{bo} ~\cite{snoek2012practical} algorithm along with a disentanglement metric called \ac{mig} \cite{chen2018isolating}. \underline{Third}, we discuss a heuristic to perform latent variable mapping to identify the set of latent variables that encodes most information of the image features. These latent variables $\mathcal{L}_d$ are used as the detector. Further, we perform a \ac{kl} based sensitivity analysis to identify the latent variable(s) $\mathcal{L}_f$ in the set $\mathcal{L}_d$, that is sensitive to specific features. The latent variable(s) in $\mathcal{L}_f$ is called reasoners and is used to identify the \ac{ood} causing features. We use the detector and the reasoners to attribute if an out-of-set feature is responsible for the \ac{ood}. The rest of this section discusses these steps.}
% }


\reviewerComment{}{Or the simulation results cannot be transferred to the real world?
}

\response{The question can be discussed in two ways. 
In the first case, if the simulation results are directly used in a real-world application, we have to make the assumption that the simulation is accurate.
In the second case, all data can be directly collected from the real world, e.g., collect data while a human driver is driving the vehicle. These data can be used as historical data to train a surrogate model or build a statistical model.
}

\reviewerComment{}{The model and implementation presented in this work are very specific for being applied to autonomous vehicles: please clarify this point since the very beginning of the paper
}


\response{We clarify that the autonomous CPS is our system of interest at the beginning of \cref{sec:ps}. However, the framework of the system is general enough to be applied to autonomous systems such as unmanned underwater vehicles and unmanned aerial vehicles. To achieve so, the environmental conditions should be updated accordingly.
}

\reviewerComment{}{Please precisely define "planning horizon" in this context.}

\response{We clarify that the planning horizon is the future scene considered during planning}

\paperQuote{{planning horizon (i.e. future scenes considered during panning)}}


\reviewerComment{}{Please precisely define "discounted cumulative reward"}

\response{The definition of "discounted cumulative reward" is that given the current state and the discounted factor, the expected return that the agent chooses the action to maximize.}


\reviewerComment{}{Tree Policy: Please better define the "current estimated value" term in the UCB equation.}

\response{need some discussion}


\reviewerComment{}{Experimental results: what does it actually mean to apply [34] from '98 to this case study? Please provide more details on the baseline used for comparison.}

\response{The baselines such as SA and GS we used for comparison all make decisions based on the same surrogate model we used in DS. The decision logics used in the prior works~\cite{phan2020neural}~\cite{johnson2016real}~\cite{desai2019soter} use conservative strategies such as switching once any unsafe state is detected. We use a similar decision logic which that maximizes the one-step reward (based on \cref{eqn:fwd}) for both SA and GS, but the conservativeness of our baselines can be tuned by changing $\alpha_1$ and $\alpha_2$. Then we perform simulations by keeping these parameters the same for SA, GS, and DS.}

\paperQuote{\textbf{Baselines}: We evaluate the performance of \ac{ds} against the following baseline controller configurations: (1) \ac{lbc} controller~\cite{chen2020learning}, (2) \ac{ap} controller~\cite{dosovitskiy2017carla}, and (3) traditional simplex architecture~\cite{seto1998simplex} with an offline decision logic for forward switching ($SA$). The forward switching is performed on the controller's historical performances, and (4) traditional simplex architecture with reverse switching ($GS$). For simplex configurations, both forward and reverse switching are performed with a myopic policy that maximizes the one-step reward (based on \cref{eqn:fwd}). }

\reviewerComment{}{Infraction score: maximum and minimum values (our lower/upper bounds) are not reported, making it hence difficult to evaluate this score. For instance, at page 7, the paper discuss a score equal to 1.0 and I found difficult to evaluate whether it is a good or a bad score. Normalized score would solve this issue.}

\response{The infraction score in the paper is already normalized to be between 0 and 1. Higher infraction score indicates the system has a better performance in safety (1 is the best, and 0 is the worst). 
}

\paperQuote{In order to evaluate safety, we compute an \textit{infraction score} as $0.5 \cdot RC + 0.25 \cdot col_{v} + 0.25 \cdot col_{o}$, where $RC$ is the percentage of the route that was completed by the vehicle, and $col_{v}$ and $col_{o}$ denote the presence of collisions with other vehicles and other objects (e.g., a wall) respectively. We design the score such that a \textbf{higher score is better}, i.e., if any infraction is observed, the resulting parameter in the score is set to 0; otherwise, it is set to 1.}

\reviewerComment{}{The experimental evaluation was performed using a hardware setup that is much more powerful that those affordable for production cars with assisted/autonomous driving features. The running times measured in this work may hence be much larger in practical settings. Please warn the reader about that.}

\response{%
We thank the reviewer for the feedback. We clarify the point in the part of discussing computation time.}

\paperQuote{\textbf{Computation Time}:
\cref{tab:computation} shows the average computation times, travel time, infraction score, and the average number of switches taken by the decision logic of our proposed $DS$ configurations. Note that the average computation time highly correlates to the computational capacity of the hardware.}


%\newpage
%---------------------------------------------------------------------
%\clearpage
\section*{Response to Reviewer \#2}

\reviewerComment{}{Given that the other (baseline) controllers are presumably not designed for handling failures, we can focus on the case when there are no failures. In this case, the proposed approach (DS) is not significantly better than the myopic switcher (GS) -- so those results by themselves do not validate the proposed approach.}

\response{%
As shown in \cref{fig:travel-safe}, the proposed DS outperforms GS in two aspects: (1) DS performs fewer switches than GS across 4 tracks. (2) DS has significantly smaller variances of infraction scores than GS on track 1 and track 3; this indicates that DS makes fewer infractions than GS.}



\reviewerComment{}{The later results on failure handling clearly show superiority of GS, but that probably indicates that GS is designed to deal to failures (whereas the baselines are not). However, DS is not presented as a way to make systems robust to failures (although it can sure be a reasonable way to do that.)}

\response{%
As the results shown in \cref{fig:failure} and \cref{fig:interfailure}, GS fails to complete the track 1, track2, and track 3 much more times than DS. This shows that DS is more robust to failures than GS.}


\reviewerComment{}{Just before start of Section 3: why use 'perf' term in forward switching? Why not just use the safety term? That brings up another issue: safety is "Boolean" and a strict constraint (rather than something that is optimized against performance) -- we typically want maximum performance subject to safety constraints. Typically, we do not want to compromise safety for perf, and that is one of the challenges with 'safety'.}

\response{%
The answer to the question is similar to the answer to how the balance is achieved for the system. We add an example in \cref{appendix:balance analysis} to explain how the system transitions happen with different scenes. Our approach is not ad-hoc to safety-critical systems but can also be applied to mission-critical systems. Depending on the goal of the system, the balance between safety and performance can be achieved by tuning the parameters in our utility functions.
}


%\newpage
%---------------------------------------------------------------------
%\clearpage
\section*{Response to Reviewer \#3}

\reviewerComment{}{Comparison with SA (forward switching Simplex) evaluates the role of backward switch, while comparison with GS (Simplex with reverse switching) evaluates the contribution of a non-myopic policy for the backward switch. These are important comparisons to make, of course. However, it is not clear to me whether SA and GS provide a fair comparison to state of the art.}

\response{%
need a discussion
}


\reviewerComment{}{The second aspect of evaluation that is missing has to do with domain rules. What is the effect of not using domain rules and just relying on MCTS for the decision? How do we evaluate whether the set of domain rules applied is sufficient? Could any of the infractions observed in experiments be avoided by having more, or different, domain rules?}

\response{%
In \cref{appendix:ablation study}, we have added the results of the ablation study in \cref{fig:ablation}. We do an ablation study in four reverse-switching configurations: myopic switch with domain rules, myopic switch without domain rules, non-myopic switch with domain rules, non-myopic switch with domain rules. Generally, domain rules are applied when the system tries to perform reverse switching while it is not in a stable state (turning) or is in a complex environment (junction). Theoretically, more and different domain rules can reduce the number of infractions, but they may also compromise the system’s performance. 
}

\section*{Response to Reviewer \#4}
\reviewerComment{}{From the presented results, it is unclear how system safety is ensured with the proposed controller.}

\response{%
We have updated \cref{sec:approach}, \cref{sec:surrogate}, and \cref{sec:conclusion} to state that the myopic selector driven by the surrogate model is an example of how to apply our approach. We’ll assume that the forward switching conditions will be provided when the approach is applied to real-world applications to guarantee safety further.
}

==> algorithms/network.tex <==
\begin{algorithm*}[!t]
    \footnotesize{}
    \caption{Neural Network Training}
	\textbf{Parameter}: Maximum game duration $T$, number of training iterations $n_i$, number of games $n_g$\\
	\textbf{Input}: Initial neural network $\mathcal{N}(S) = [P,V]$, initial state $S_1 = [s_{c,1},s_{e,1},s_{v,1},r_1]$, reward function $R(S_t)$, action selection function $A(\pi_t,\pi_{t-1})$\\
	\textbf{Output}: Trained neural network $\mathcal{N}$
	\begin{algorithmic}[1]
	\State Initialize empty training data set $D$
	    \For{$g=1,2,...,n_g$}
	        \State Initialize simulation with initial state $S_1$
	       \For{$t=1,2,...,T$}
	            \State Run controller $c_t$ specified by $s_{c,t}$
	            \State Observe and store reward $R_{t}$ 
	            \If{$t = T$ or $R_t = -1$}
	                \State Calculate accumulated reward $R_{total} = \sum_{i=1}^{t}R_i$
	                \State Create $t$ new training data points $d_{new,i} = \{S_i,\pi_i,R_{total}\}$, $i \in \{1,2,...,t\}$
	                \State Break
	            \EndIf
	            \State Run \ac{mcts} on state $S_t$ to obtain policy $\pi_t$
	            \State Evaluate $A(\pi_t,\pi_{t-1})$ and get new controller state $s_{c,t+1}$
	            \State Observe environment and vehicle state to get new states $s_{e,t+1}$ and $s_{v,t+1}$
	            \State Calculate new risk $r_{t+1}$
	        \EndFor
	    \State Append new training data to training set: $D = D \cup \{d_{new,i} | i \in \{1,2,...,t\} \}$
	    \State Retrain $\mathcal{N}$ with training data $D$ for $n_i$ iterations
	\EndFor
	\end{algorithmic} 
	\normalsize{}
\label{algo:alphazero_network}
%\vspace{-0.05in}
\end{algorithm*}

==> algorithms/selector-new.tex <==
\begin{algorithm}[!t]
    \footnotesize{}
    \caption{Controller Selection}
	\textbf{Parameter}: neighborhood size $k$\\
	\textbf{Input}: \ac{lut} data $X_{input}$, travel route $srout$, current state $s_i$, current location $sloc$  \\
	\textbf{Output}: $p(C^p|s_i)$, $p(C^s|s_i)$
	\begin{algorithmic}[1]
	\State $X_{sub}$ $\longleftarrow$ generate\_clusters($X_{input}$,$r$) \Comment{generate data clusters}
	\State $X_{cluster}$ $\longleftarrow$ $X_{sub}[sloc]$ \Comment{match the cluster}
	\For{$x$ in $X_{cluster}$}      \Comment{search within cluster entries}
	    \If{$c^f_i$ in $x$}
            \State $X_{sel}$ $\longleftarrow$ $x$
        \EndIf
    \EndFor
    \If{$s_i[f^t]$ in $X_{sel}$}
        \State \Return  $p(C^p|s_i)$, $p(C^s|s_i)$
    \Else
        \State Neighbors ($N$) $\longleftarrow$ KNN($s_i[f^t]$,${X}_{sel}$,$k$)
        \State T1 $\longleftarrow$ [], T2 $\longleftarrow$ [] 
        \For{$n \in N$}
            \State $p(C^p)$,$p(C^s)$ $\longleftarrow$ get\_score($X_{sel}[n]$) \Comment{get beliefs}
            \State T1.append($p(C^p)$, T2.append($p(C^s)$
        \EndFor
	    \State $p(C^p|s_i) \longleftarrow sum(T1)/len(T1)$ \Comment{average belief}
	    \State $p(C^s|s_i) \longleftarrow sum(T2)/len(T2)$
    \EndIf
    \State \Return $p(C^p|s_i)$, $p(C^s|s_i)$ 
	
% 	 \Function {generate\_clusters}{$X_{input}$,$r$} 
% 	    \State $X_{sub}$ $\longleftarrow$ [] 
% 	    \For{$f^s \in r$} 
%             \For{$x \in X_{input}$}
%                 \State $T$ $\longleftarrow$ []
%         	   \If{$f^s$ == $x[f^s]$} \Comment{check structural feature similarity}
%         	        \State $T$.append($x[f^s]$, $x[p(C^p)]$, $x[p(C^s)])$
%         	   \EndIf
%         	 \State $X_{sub}$.append($T$)
%         	\EndFor
%   \EndFor
%     \State \Return $X_{sub}$
%     \EndFunction
	\end{algorithmic} 
	\normalsize{}
\label{algo:selector}
%\vspace{-0.05in}
\end{algorithm}

==> algorithms/selector.tex <==
\begin{algorithm}[!t]
    \footnotesize{}
    \caption{Controller Selection}
	\textbf{Parameter}: neighborhood size $k$\\
	\textbf{Input}: pre-processed controller \ac{lut} data $X_{input}$, current sensor failure state $S^F_i$, current structural $\mathcal{S}_i$ and temporal labels $\mathcal{T}_i$,  \\
	\textbf{Output}: $p(C_p|scene,S^F)$, $p(C_s|scene,S^F)$
	\begin{algorithmic}[1]
	\For{$x \in X_{input}$}
	   \If{$x[\mathcal{S}]$ == $\mathcal{S}_i$}
	        \State $X_{sub}$ $\longleftarrow$ $x[\mathcal{T}, p(C_p), p(C_s)]$
	   \EndIf
   \EndFor
   \If{$\mathcal{T}_i$ in $X_{sub}$}
        \State \Return  $p(C_p|scene,S^F), p(C_s|scene,S^F)$
    \Else
        \State Neighbors ($N$ $\longleftarrow$ KNN($\mathcal{T}_i$,$\mathcal{X}_{sub}$,$k$)
        \For{$n \in N$}
            \State $p(C_p)$,$p(C_s)$ $\longleftarrow$ get\_score($X_{sub}[n]$)
            \State scores $\longleftarrow$ $p(C_p)$, $p(C_s)$
        \EndFor
	    \State Compute the average $p(C_p)$, $p(C_s)$ scores
        \State \Return $p(C_p|scene,S^F)$, $p(C_s|scene,S^F)$
	    \EndIf
	\end{algorithmic} 
	\normalsize{}
\label{algo:selector}
%\vspace{-0.05in}
\end{algorithm}

==> algorithms/switching.tex <==
\begin{algorithm}[!t]
    \footnotesize{}
    \caption{Controller Switching}
	\textbf{Parameter}: switching speed $\tau_s$\\
	\textbf{Input}: current state $s_i$, current location $sloc$, current speed $v$ \\
	\textbf{Output}: $control\_action$
	\begin{algorithmic}[1]
   \If{$C^d$ == $C^p$}
        \State $a_i \longleftarrow Selector(s_i)$ \Comment{run selector}
        \State $control\_action$ $\longleftarrow$ $routine$(v,$\tau_s$,$a_i$)
   \ElsIf{$C^d$ == $C^s$}
        \State $a_i \longleftarrow Planner(s_i)$ \Comment{run planner}
        \State $control\_action$ $\longleftarrow$ $routine$(v,$\tau_s$,$a_i$)
    \EndIf
    \State \Return $control\_action$
    
    % \Function {routine}{v,$\tau_s$,$a_i$}
    % \If{$sloc \in acceptable\_areas$} \Comment{domain-specific rule check}
    %     \If{$a_i == switch$}
    %         \If{v $>$ $\tau_s$}
    %             \State $control\_action$ = decrease speed
    %         \ElsIf{v $\leq$ $\tau_s$}
    %             \State $control\_action$ = no change 
    %         \EndIf
    %     \EndIf
    % % \Else
    % %     \State $control\_action$ = no change 
    % \EndIf
    % \State \Return $control\_action$ \Comment{control action for the system}
    % \EndFunction
	\end{algorithmic} 
	\normalsize{}
\label{algo:switching}
%\vspace{-0.05in}
\end{algorithm}

==> sections/approach.tex <==
\section{Dynamic Simplex Strategy}
\label{sec:approach}

\begin{figure}[t]
 \centering
 \includegraphics[width=\columnwidth]{figures/transition.png}
 \caption{Controller transitions caused by different decision events. $C^P$ and $C^s$ respectively indicate performant controller and safety controller. Once a decision event occurs, the decision-maker takes time to decide whether a switching must be performed. In the case of a forward switch, the selector takes $t_s$ seconds to decide, and in the case of a reverse switch, the planner takes $t_p$ seconds to make the decision.}
 \label{fig:example-transition}
 \vspace{-0.1in}
\end{figure}

We show an overview of our dynamic simplex strategy in \cref{fig:overview}. To perform the switching decision, the strategy has the following components. (1) the switcher we model as an SMDP decides ``if" and ``when" the switching must be performed. For deciding if a switch is required, at the occurrence of a \textit{decision event} (refer to the problem formulation), the switcher queries one of the following decision-makers: (a) the selector for a forward switch in case the performant controller is driving the system, or (b) the planner for a reverse switch in case the safety controller is driving the system. In implementing these components, we assume the availability of a map that can provide the route the system will travel and its current location on the route. We also assume access to a \ac{lut} with historical performance (speed) and safety (collisions) information of the two controllers. 

% The occurrence of one or more of the following decision events triggers the switcher because it will change the state of the system. First, in case the system enters a new scene (as scenes are typically 15 to 30 seconds long, the system frequently enters new scenes). That is if the weather or the spatial features (road curvature and type of road) change. Second, if one or more components (sensors and actuators) fail, the onboard runtime monitor raises the alarm. In implementing these components, we assume the availability of a map that can provide the route the system will travel and its current location on the route. We also assume access to a \ac{lut} with historical performance (speed) and safety (collisions) information of the two controllers. 

\cref{fig:example-transition} shows a controller transition diagram with the decision events occurring at different times (highlighted in red). On the occurrence of a decision event, the switcher works as follows. It first checks for the controller driving the system. If the performant controller is operating the system, the switcher activates the selector, which takes $t_s$ seconds to decide if the switch is required or not. For this, it searches a \ac{lut} with prior beliefs on the controller's performance and computes the reward for each controller using \cref{eqn:fwd}. No switching is performed if the performant controller has a higher reward. Otherwise, a forward switch is performed. Next, if the safety controller is operating, the switcher activates the planner, which takes $t_p$ seconds to decide if a reverse switch is required. For this, it uses a generative model to simulate different weather conditions for the $n$ scenes in the future using \ac{mcts}. It performs a tree search that returns if a switch to the performant controller is worthy of being executed. However, if a new decision event occurs while either decision-maker is processing, the decision process will be terminated and initiated with the new state. We describe each decision-making component in greater detail in the rest of this section. 

% Finally, the actions selected by the decision-makers are sent to the switcher. If the returned action involves switching, the switcher activates a controller transition routine to start the control transition process (discussed in the following section). We describe each decision-making component in greater detail in the rest of this section. 

\subsection{Switcher}
As discussed, the switcher is activated when a \textit{decision event} occurs. Depending on the kind of events affecting the system's safety, one or more monitors must be designed to detect these events at runtime. While we do not prescribe specific monitors, we leverage our previous work on runtime monitors~\cite{kuhn2020introspective,ramakrishna2022risk}; the implementation details are presented in the evaluation section. 

% Depending on the events increasing the system's risk, we will need to include one or more runtime monitors. Our approach does not demand custom monitors. So, we can utilize an existing monitor based on the decision events of interest. We leverage our previous work on runtime monitors~\cite{kuhn2020introspective,ramakrishna2022risk}; the implementation details are presented in the evaluation section. 

Next, once these onboard monitors detect an event (change in weather, scenes, or component failures), the switcher selects an action as illustrated in \cref{algo:switching}. If the performant controller is driving the system and the selector chooses to use the safety controller, the switcher will prepare to switch the system's control to the safety controller. However, if the safety controller is operating and the planner chooses to use the performant controller, the switcher will prepare to switch to the performant controller. If the decision-maker decides not to switch, the switcher will continue using the current controller. 


% \begin{equation}
% a_i =
% \begin{cases}
%   C^p \longrightarrow C^s, & \text{if}\ Selector(s_i) = C^s \\
%   C^s \longrightarrow C^p, & \text{if}\ Planner(s_i) = C^p \\
%   a_{i-1}, & otherwise
% \end{cases}
% \label{eqn:switcher}
% \end{equation}
A switching routine is activated if the decision-maker decides to switch the current driving controller. Instead of an instantaneous controller transition, the routine will consider the system's physical state and domain-specific rules to determine when and how the control transition must be performed. For this, it will first trigger a slow change in the control action (e.g., reduce speed). The change in the control actions is performed when: (a) the system's current speed ($v$) $<$ switching speed ($\tau_s$), and (b) the system is operating within the acceptable areas prescribed by our domain-specific rules. That is, we have a set of rules describing where the switching can be performed. For example, some acceptable areas for switching include the main road, overpass, and freeway. Rules for no switching include intersections, lane changes, or roundabouts. The routine will perform the controller transition when both these conditions are satisfied. 

Also, to avoid the excessive burden of computation caused by running both controllers in parallel, the switcher warms up the controller selected by the decision-maker before bringing it online during this transition phase. Accordingly, the switcher routine will start operating the selected controller in a shadow mode by sending it sensor data for predicting the control actions, which are discarded until the completion of the transition phase. After the transition phase is completed, the selected controller's predictions start being used for operating the system.

\input{algorithms/switching}



% to perform the control transition. Specifically, it will trigger a change in the control action that the system will need to complete to accommodate the switch. In case of no switch, the switcher will not suggest any change in the control actions. However, in the case of a switch, the routine checks for two conditions: First, the current speed of the system. Suppose the system's current speed ($v$) $>$ switching speed ($\tau_s$), the switcher will suggest the system reduce its speed. The second is a set of domain-specific rules describing where the switching can and cannot be performed. These rules are mainly based on location and operating context. For example, some acceptable areas for switching include the main road, overpass, and freeway. Rules for no switching include intersections, lane changes, or roundabouts. If both these conditions are satisfied, the switcher performs a switch to the selected controller.

% the belief of the performant controller $p(C^p|s)$ in the given state $s$, and the belief of the safety controller $p(C^s|s)$ in the given state $s$. 

\subsection{Selector}
\label{sec:selector}
When activated, the selector searches a \ac{lut} to select an optimal controller for the current state based on its historical performances. The table includes the scene\_label of the given state $s$ and the prior beliefs of the controllers in the given state $s$. The belief represents the best rationale assessment of the controller


To get the beliefs, we run a search on the table using the \ac{knn}~\cite{friedman1975algorithm} algorithm. However, searching the entire table may get expensive if it contains many entries. To speed up the search, we first cluster the entries into distinct groups based on the structural scene labels $f^s$ of the system's travel route $srout$. Then, we select one cluster based on the system's current location $sloc$ (assumed to be available from a GPS sensor). 

The search within the cluster is shown in \cref{algo:selector}, and it works as follows: We separate the cluster entries further into two groups. The first group has entries where a sensor failure occurred, and the second group has entries where no failures occurred. Then, we apply the \ac{knn} algorithm to one of these groups based on the occurrence of a failure or not (information available from the onboard monitors). The goal of the search is to find the $k$ nearest entries in the cluster that matches the weather conditions of the current scene\_label. The controller's performance in the selected neighbors is averaged to get the controller's belief. These scores are used to compute the reward (see \cref{eqn:fwd}), which is used to decide if a forward switch is required or not.

\input{algorithms/selector-new}

\subsection{Planner}
When activated, the planner takes the current state as the input and returns if a reverse switch is required by looking into the near future. For this, it simulates the possible future operating conditions and system's component failures using the \ac{mcts} online algorithm. Since the operating conditions and the component failures vary dynamically, using an online algorithm is a natural choice. 

\ac{mcts} is a heuristic search algorithm for finding optimal decisions in a decision space by build a search tree~\cite{browne2012survey}. The tree nodes represent the states, and the edges represent the actions that mark the state transitions. The search begins with a root node, and a child node is recursively selected until a leaf node is reached. Unless this leaf node denotes the end of the planning horizon, an action is taken in this state node, and the tree is expanded by adding corresponding child nodes. To estimate the value of an action from a node, the algorithm simulates a ``rollout" from the child node to the end of the planning horizon with a computationally cheap default policy. Using the algorithm requires three components: (1) generative model to simulate the future states, (2) tree policy to navigate the tree search, and (3) default policy to estimate the value of an action. We describe these components below.  

% The tree can be explored asymmetrically to search for the actions with the most promising rewards.

\textbf{Generative Models}: As discussed, we use a set of generative models to perform the state transition. The weather model provides a method for sampling new weather conditions as the tree is built. The sensor failure model provides a method for sampling different sensor failures. We learn the weather model based on the historical data gathered from many previous simulations. We primarily learn the rate at which the different weather parameters vary. Similarly, we use the sensor failure rate and severity to build the sensor failure model. For example, a digital camera's failure rate is roughly 0.1\% over $2$ years of operation. While some of these failures (e.g., bright images) get rectified over time, other failures (e.g., broken lens) persist until replacement.  

\textbf{Tree Policy}: We employ the tree policy for searching the tree and deciding which nodes must be visited. The action selection in the policy is driven by the standard Upper Confidence bound for Trees (UCT)  algorithm~\cite{KocsisS06}, which defines the score of a node as

\begin{equation}
    UCB(s,a) = Q(s,a) + c_{uct} \sqrt{\frac{\ln{N(s)}}{N(s,a)}}
\end{equation}
Where, $Q(s,a)$ is an estimated value for taking the action $a$ in the state $s$, $N(s,a)$ denotes how often the action $a$ has been taken in the state $s$, $N(s)$ is the number of times $s$ has been visited, and $c_{uct}$ is used to tune the trade-off between exploration and exploitation. A higher value for $c_{uct}$ puts less emphasis on the current value estimation $Q(s,a)$ and forces the tree towards actions taken less frequently. The first term $Q(s,a)$ is the exploration term that biases the search toward the nodes which appear promising. The second term is the exploitation term which encourages the attempts at the under-represented action for the current state.

\textbf{Default Policy}: We employ a default policy to estimate the value of action during rollout. Our default policy is random. We randomly select an action that should be taken when the safety controller is operating the system. If the chosen action is ``to switch" to the performant controller, we will sample the future state only from a set of states with the driving controller as the performant controller. The idea behind biasing the sampling process is that we want to see how the expected rewards will be if the system continues using the performant controller in the future.

% \textbf{Search Policy}: We employ two policies during the tree search. The first is the tree policy for searching the tree and deciding which nodes must be visited. The action selection in the policy is driven by the standard upper confidence bound for trees (UCT)  algorithm~\cite{KocsisS06}. Next, we employ a default policy to estimate the value of action during rollout. Our default policy is random. We randomly select an action that should be taken when the safety controller is operating the system. If the selected action is to switch to the performant controller, then we will sample the future state from a reduced state space which has the driving controller to be the performant controller. The idea behind biasing the sampling process is that we want to see how far in the future the system can use the performant controller once the reverse switch has occurred.  
% use random action selection to decide which action should be taken when the safety controller is operating the system. Once the action indicates the controller should be switched to the performance controller, the system would stay with the performant controller until the end of the rollout. Our idea behind the random selection is that we want the control to remain with the performant controller as long as possible once the reverse switch has occurred. 

\input{algorithms/mcts}

\textbf{Tree Search}: The tree search algorithm is shown in \cref{algo:mcts}. Given that we are simulating the future operating conditions, running the tree search once does not adequately represent the future conditions. To handle this, we run the tree search for multiple iterations, which gives us more comprehensive coverage of the possible conditions. The search begins each iteration by initializing the current state $s$ as the tree's root node. If the current state is the tree's terminal state (leaf node), then the reward for this state is calculated, and the search for this iteration is terminated. We use the \ac{knn} algorithm, discussed in \cref{algo:selector} to get the performance and safety scores and combine it with the switch counts to compute the reward using \cref{eqn:rev}. 

If the current state was not visited during the earlier search, a rollout is performed from the current state node by randomly selecting actions until a leaf node is reached. The simulation outcome is then propagated back to the root node while averaging the rewards (see \cref{eqn:rev}). However, if the state was visited earlier, an action that maximizes the \ac{ucb} is selected. Then, based on this action, the generative models simulate a new state, which then becomes the root node of a new tree search. Finally, a backward pass is performed to update the Q-value $Q(s,a)$ and the visit count of all the previous nodes visited during the iteration.

==> sections/background.tex <==
\section{Background}
\label{sec:background}
In this section, we introduce the key theory required for the proposed approach: \ac{mdp}, and \ac{mcts}.

% \subsection{Controller Redundancy Architectures}

% Simplex Architecture~\cite{bodson1994analytic,seto1998simplex}, controller sandboxing~\cite{bak2011sandboxing}, and controller blending~\cite{gohari2020blending} are different architectures that provide controller redundancy for software fault tolerance and safety assurance of \ac{cps}. The redundancy is achieved by augmenting different controllers to the system and then selecting which one is most appropriate for driving the system. Typically, these architectures have a primary high performant controller ($C_p$), a secondary safety controller ($C_s$), and a decision logic. 

% The DM hosts a logic to select a controller based on the desired objective of the system. Safety and performance are the two main objectives that the logic needs to optimally balance while selecting the controller. The key challenge with these architectures is to create the decision logic. A conservative logic would always use the safety controller, delaying or ignoring the mission-critical objectives of the system. However, switching the control tool late would not give sufficient time for the system to recover~\cite{johnson2016real}. Also, once the logic switches to the safety controller, the control remains with it forever in these architectures. There is relatively little work on reverse switching from the secondary controller to the primary~\cite{johnson2016real,desai2019soter,phan2020neural}. 

% The authors in~\cite{desai2019soter} use reachability analysis to determine the system's safety in the subsequent two inference cycles before making the reverse switching. Jonhson \emph{et al.}~\cite{johnson2016real} consider the system's stability in performing the reverse switch. In Neural Simplex Architecture~\cite{phan2020neural}, the authors present two reverse switching strategies. The first strategy looks to the near future to check a forward switch will not occur in a short time. The second one performs the forward switch when the logic decides the system is sufficiently safe. In this work, we perform the reverse switching using a planner that estimates the system's future risk from the performant controller in possible operating conditions. The future risk determines if the reverse switch needs to be performed or not.

% A \ac{mdp} is a generalization of the MDP and is applicable when the state of the environment is not directly observable~\cite{kaelbling1998planning}.

\subsection{Markov Decision Process}
An \ac{mdp} is a mathematical framework for modeling sequential decision making process in a stochastic environment. It is defined as a tuple $\langle S,A,T,R \rangle$, where $S$ is the set of environment states, $A$ is a set of actions that the agent can perform, $T$ is the state transition model, and $R$ is the reward function. The transition model $T(s,a,s')$ = $Pr(s'|s,a)$, describes the probability of executing an action $a$ from a state $s$ to transition to state $s'$. The goal of the agent at every time step $t$ is to select an action $a$ from $A$ that maximizes the future discounted reward $R_n$ computed as:

\begin{equation}
 \sum_{t=0}^{\infty} \gamma^t \cdot r_t  
 \label{eqn:reward}
\end{equation}

Where, $r_t$ is the immediate reward received by the agent at step t, $\gamma \in [0,1]$ is the discount factor that determines if the agent cares about the current reward or the future reward. With $\gamma = 0$, the agent is myopic and only cares about optimizing the current reward, and with $\gamma = 1$, the agent only cares of the future reward. An intermediate value is needed to balance the current and future rewards.   
  
\subsection{Monte Carlo Tree Search}
\ac{mcts} has become a de-facto standard for solving \acp{mdp}. It is an online heuristic search algorithm for finding approximately optimal decisions by randomly sampling in the decision space to build a decision tree~\cite{browne2012survey}. 
The idea of \ac{mcts} is to construct a search tree consisting of both state and action nodes until some predefined budget (e.g., time or resource) is reached. When an action in a state node is taken, the tree is expanded by adding a corresponding action node to the tree. The goal is to estimate the function $Q(s, a)$ that assigns each state-action pair a value. This value corresponds to the expected return $r_t$ that taking the action $a$ in the current state $s$ would lead to eventually. To obtain future states in each tree search, a generative model $G(s,a)$ is used. For selecting an action in the current state, the upper confidence
bound (UCB) can be used, given as

\begin{equation}
    UCB(s,a) = Q(s,a) + c \sqrt{\frac{\ln{N(s)}}{N(s,a)}}
\end{equation}

$N(s,a)$ denotes how often the action $a$ has been taken in the state $s$. To tune the trade-off between exploration and exploitation, the parameter $c$ is used. A higher value for $c$ puts less emphasis on the current value estimation $Q(s,a)$ and forces the tree towards actions which are taken less frequently. A more comprehensive introduction to \ac{mcts} can be found in~\cite{browne2012survey}.

\begin{figure*}[t]
 \centering
 \includegraphics[width=0.8\textwidth]{figures/workflow3.pdf}
 \caption{Overview of the proposed decision logic for controller redundant architecture. Based on the runtime monitor results, the selector queries the controller \ac{lut} to get the prior belief on the controller's performance and selects a suitable controller. The switcher then decides if and when to switch and uses the planner to perform reverse switching.}
 \label{fig:overview}
\end{figure*}
